SAGE: Saliency-Guided Mixup with Optimal Rearrangements

Data augmentation is a key element for training accurate models by reducing overfitting and improving generalization. For image classification, the most popular data augmentation techniques range from simple photometric and geometrical transformations, to more complex methods that use visual saliency to craft new training examples. As augmentation methods get more complex, their ability to increase the test accuracy improves, yet, such methods become cumbersome, inefficient and lead to poor out-of-domain generalization, as we show in this paper. This motivates a new augmentation technique that allows for high accuracy gains while being simple, efficient (i.e., minimal computation overhead) and generalizable. To this end, we introduce Saliency-Guided Mixup with Optimal Rearrangements (SAGE), which creates new training examples by rearranging and mixing image pairs using visual saliency as guidance. By explicitly leveraging saliency, SAGE promotes discriminative foreground objects and produces informative new images useful for training. We demonstrate on CIFAR-10 and CIFAR-100 that SAGE achieves better or comparable performance to the state of the art while being more efficient. Additionally, evaluations in the out-of-distribution setting, and few-shot learning on mini-ImageNet, show that SAGE achieves improved generalization performance without trading off robustness.

==> discussion.tex <==
In Table~\ref{table:classification_accuracy}, we summarize the testset accuracy of models trained using different DA approaches. 
% 
Comparing to the two other saliency-based method, models trained using \Ours{} is slightly behind.
% 
This is because Puzzle and Co-mix both involve solving an additional optimization problem to further maximize the saliency of the resulting mixed images.
% 
From a high level, it allows images to be mixed with an offset.
% 
% With such an offset, 
In Input mixup and \Ours{}, pixel locations in both images are fixed, meaning no horizontal nor vertical translation of the images are allowed.
% 
In Puzzle and Co, when two images are shifted and mixed together to maximize saliency, the resulting image resembles moving the slient region from one the first image to cover the non-salient region in the second image.
% 
Through this process, the resulting image keeps the most salient parts from both images.
% 

Such an mixing strategy in Puzzle mix and Co-mix introduces an extra degree of freedom compared to conventional styles of mixup such as Input Mixup and \Ours{}.
% 
As such, we believe that having this extra degree of freedom could potentially further improve our method.

\paragraph{Ideas...}
One computationally simple way is to use the concept of region proposals in Faster-RCNN\citep{}, and mix the two saliency map based on a set of predefined offsets, and pick the one that maximizes the resulting saliency. Finally, the two images are mixed based on the saliency map and the offset that maximizes the saliency.



==> rebuttal.tex <==
\setlength\parindent{0pt}
% We are thankful to the reviewers for their comments. We will fix/revise all minor issues, including ...
%We thank the reviewers for their feedback and positive ratings. We are glad \textbf{R1} find our method \blue{novel} and the paper \blue{clearly written}, \textbf{R3} describes our method as \blue{``efficient''}, and \textbf{R4} finds it \blue{``simple and well motivated''}. Below, we respond to all reviewers' questions and concerns.
We thank the reviewers for their feedback and positive ratings. We are pleased that the reviewers find the paper \blue{``clearly written''} (\textbf{R1}), and our method \blue{``novel''} (\textbf{R1}), \blue{``efficient''} (\textbf{R3}), and \blue{``simple and well motivated''} (\textbf{R4}). Below, we respond to all reviewers' questions and concerns.

\textbf{R1/R4:}
\blue{Improvements on image classification are marginal.}
\\
The absolute improvement with respect to the vanilla classification model is consistent and significant in all the setups.
While in some cases the improvement may be marginal with respect to the other data augmentation techniques, our method is more efficient and does not sacrifice OOD generalization, which is a significant advantage on its own.
% 
% Note that the main advantage of the proposed method is the significantly shortened training time and improved generalization performance in the OOD setting while maintaining similar or better standard classification accuracy.
% 
\\
\textbf{R1:}
\blue{Insufficient OOD experiments.}
To show OOD generalization beyond adversarial attacks, we compare SAGE to other data augmentation techniques for few-shot classification on mini-ImageNet, where the goal is to learn a representation that generalizes to novel categories.
We follow the setup of~[A], using a single ResNet12 with the prototype classifier.
As Tab.~\ref{table:few-shot} shows, \Ours{} outperforms other augmentation techniques, including MixUp (the strongest model on adversarial perturbations). 
This shows that \Ours{} is useful in OOD scenarios beyond adversarial perturbations.
We will include this result in the final manuscript.
\blue{Difference with SaliencyMix.}
We thank the reviewer for pointing out this work.
While SaliencyMix somewhat resembles our SAGE, the two methods differ significantly at the conceptual level.
First, SAGE formulates the data augmentation as saliency maximization that leads to more diverse samples, whereas SaliencyMix merely uses saliency to swap-out informative image regions.
Second, SAGE uses smooth mixing masks spanning entire images, while SaliencyMix uses small binary masks resulting in patch-like augmentations (like CutMix, Puzzle Mix and Co-Mixup).
Consequently, SaliencyMix shows inferior robustness performance, see Fig.~\ref{fig:comparison}.
Third, SaliencyMix requires an external trained saliency detector (i.e., they use a shallow pre-deep-learning method), while SAGE repurposes the gradients of the CNN backbone to compute the saliency maps.
% computes saliency using a shallow pre-deep-learning method, that mostly ignores image semantics and is inferior to deep methods (used in SAGE).
Empirically, the classification performance does not match that of SAGE, as shown in Tab.~\ref{table:classification_accuracy}.
\blue{Discrepancy in robustness evaluations compared to the reported results in SaliencyMix~[B].}
% Several factors could lead to such differences. 
% 
Our experimental setup (model selection, training objective and optimization schedule) is identical to the ones used in previous work~[10, 11, 19], which slightly differs from that of SaliencyMix.
To measure the robustness and cover a wide variety of OOD settings, we report the average accuracy across three types of common perturbations (Ln.\ 319)
On the other hand, results reported in SaliencyMix only focus on the $\ell_{\inf}$-norm FGSM, which is a key source of the discrepancy.
At the same time, our FGSM results (in the Supplement) are consistent with that of CutMix (in Tab.\ 2,3 of [10]).
The other differences between our setup (following [10, 11, 19]) and SaliencyMix include:
(i) the base model, i.e., we use the PreActResNet 
rather than the vanilla ResNet (we will clarify this point in the paper);
(ii) the training loss, i.e., we use Binary Cross Entropy rather than Cross Entropy.
% We follow the setup in~[10, 11, 19] for both choices.

\begin{figure}[t]
% \captionsetup[subfigure]{labelformat=simple}
\centering 
% \subfloat[Robustness Comparison]{\label{fig:robustness_comparison}
\includegraphics[width=.95\linewidth]{figure/rebuttal-robustness-cifar100.pdf}
\\
\vspace{-5pt}
% \subfloat[Runtime Comparison]{\label{fig:runtime_comparison}
\includegraphics[width=.95\linewidth]{figure/rebuttal-runtime-cifar100.pdf}
\vspace{-10pt}
\caption{
\textbf{Robustness (top) and efficiency (bottom) analysis of \Ours{}.} (including additional comparisons with SaliencyMix) 
% (a) Robustness versus standard accuracy in OOD generalization. 
% The methods in the green area (i.e., Mixup and \Ours{}) improve both accuracy and robustness relative to vanilla augmentation, while the others in red (i.e., CutMix, SaliencyMix, Co-Mixup and Puzzle Mix) improve standard test accuracy at the cost of decreased robustness.
% (b) Runtime comparison of SAGE and other baselines. 
% We estimate computation cost with a single NVIDIA Tesla T4. For SAGE, there is no noticeable overhead besides the additional forward and backward pass to compute the saliency map which approximately doubles the time of Vanilla training.
}
% \label{fig:cifar100_runtime_robustness_comparison}
\label{fig:comparison}
\vspace{-10pt}
\end{figure}

\begin{table}[t]
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{2mm}
\small
\begin{tabular}{ lllllllll } 
Dataset & Model         & Mixup & SaliencyMix       & \Ours{} \\
\Xhline{2\arrayrulewidth}
CIFAR-10   & ResNet18   & 95.97 & 96.15      & \textbf{96.95} \\ 
CIFAR-100  & ResNet18   & 77.40 & 78.85      & \textbf{79.91} \\ 
CIFAR-100  & WRN16      & 79.83 & 80.16      & \textbf{80.45} \\ 
CIFAR-100  & ResNext29  & 78.23 & 78.89      & \textbf{80.35} \\
\Xhline{2\arrayrulewidth}
\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\caption{\textbf{Image classification accuracy.} 
% CIFAR-10 and CIFAR-100 results are obtained by averaging over three independent training runs.
}
\label{table:classification_accuracy}
\vspace{-10pt}
\end{table}

\begin{table}[t]
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{2mm}
\small
\begin{tabular}{ cccccccccc } 
Vanilla & CutMix  & Mixup &  Puzzle  & Co-Mixup & \Ours{} \\
\Xhline{2\arrayrulewidth}
77.9   & 78.4   & 78.9 & 78.6  & 79.0    & \textbf{79.8} \\ 
\Xhline{2\arrayrulewidth}
\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\caption{\textbf{Few-shot classification accuracy on mini-ImageNet.}}
\label{table:few-shot}
\vspace{-18pt}
\end{table}

\textbf{R3:} \blue{The mechanism of selecting $\zeta$.}
We clarify that the role of $\zeta$ in Eq.2 is for computation stability, i.e., avoiding division-by-zero, and in fact does not affect the creation of the realistic images. We will clarify this point.
\\
\textbf{R4}: \blue{What classifier is used to compute the saliency?}
At each iteration, we use the current partially trained model to compute the saliency (Ln.\ 147), which is more computationally efficient (Ln.\ 264) and convenient.
We will emphasize this in the paper.
\blue{The experimental evaluation relies on rather small datasets.}
Experiments on CIFAR10 and CIFAR100 are standard and allow direct comparison to existing literature~[10, 11, 19].
While we agree that experimenting with large-scale datasets like ImageNet may further benefit the work, as suggested by R4 the required computational resources are out of scope for us.
% We thank the reviewer for understanding.
\blue{Every page of the paper is a Figure.}
We thank the reviewer for pointing out this issue.
To mitigate it for now, we re-upload Fig.~\ref{fig:comparison} (with the included comparison to SaliencyMix).

\textbf{References:}\\
$[\text{A}]$ Dvornik et al., Diversity with cooperation: Ensemble methods for few-shot classification, ICCV 2019\\
$[\text{B}]$ Uddin et al., SaliencyMix: A saliency guided data augmentation strategy for better regularization, ICLR 2021


